Alternate Groundwater Modelling Strategies: A Multi-Faceted Data-Driven Approach

The impact of statistical methodologies on studying groundwater has been significant in the last several decades, due to cheaper computational abilities and presence of technologies that enable us to extract and measure more and more data. This paper focuses on the validation of statistical methodologies that are in practice and continue to be at the earliest disposal of the researcher, demonstrating how traditional time-series models and modern neural networks may be a viable option to analyze and make viable forecasts from data commonly available in this domain, and suggesting a copula-based strategy to obtain directional dependencies of groundwater level, spatially. This paper also proposes a sphere of model validation, seldom addressed in this domain: the model longevity or the model shelf-life. Use of such validation techniques not only ensure lower computational cost while maintaining reasonably high accuracy, but also, in some cases, ensure robust predictions or forecasts, and assist in comparing multiple models.

==> table_1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet8'
\begin{table}[htbp]
  \centering
  \caption{List of groundwater stations between which copula directional dependence was found to be greater than 0.95}
    \begin{tabular}{|c|c|c|c|}
    \hline
    \multirow{1}{*}{\textbf{Station 1 ($U$)}} & \multirow{1}{*}{\textbf{Station 2 ($V$)}} & \multirow{1}{*}{\textbf{$\rho_{U \rightarrow V}$}} & \multirow{1}{*}{\textbf{$\rho_{V \rightarrow U}$}} \\
      \hline
    Alladpur & Chisadia & 1     & 0.94683 \\
    \hline
    Alladpur & Segwa Chowki I & 0.96587 & 0.9674 \\
    \hline
    Amreshwar & Handod I & 0.96479 & 0.96443 \\
    \hline
    Amreshwar & Makni & 0.97426 & 0.974 \\
    \hline
    Amreshwar & Segwa Chouki II & 0.98572 & 0.98474 \\
    \hline
    Amreshwar & Vadodara II & 0.96374 & 0.96193 \\
    \hline
    Asala & Chitral PZ II & 0.97568 & 0.9752 \\
    \hline
    Baladgam & Makni & 0.95694 & 0.95908 \\
    \hline
    Bhindol & Kosindra Pz I & 0.99311 & 0.9933 \\
    \hline
    Bhindol & Pitha & 0.96079 & 0.96143 \\
    \hline
    Bhindol & Vadtalav PZ & 0.97362 & 0.97328 \\
    \hline
    Bodeli & Kosindra PZ I & 0.96573 & 0.96685 \\
    \hline
    Chisadia & Panwad & 0.9631 & 0.96486 \\
    \hline
    Chitral PZ II & Makni & 0.99218 & 0.99237 \\
    \hline
    Chitral PZ II & Vadodara I & 0.96172 & 0.96216 \\
    \hline
    Devat (Thadgam) & Saidivasana & 0.95406 & 0.96142 \\
    \hline
    Ghayaj II & Makni & 0.99612 & 0.99629 \\
    \hline
    Handod I & Karamasiya & 0.95198 & 0.95206 \\
    \hline
    Handod I & Segwa Chouki II & 0.98175 & 0.98154 \\
    \hline
    Handod I & Vadodara I & 0.95313 & 0.95351 \\
    \hline
    Kaprali & Pitha & 0.97459 & 0.97362 \\
    \hline
    Karamasiya & Kosindra PZ I & 0.95942 & 0.95911 \\
    \hline
    Pavi  & Vadtalav PZ & 0.97843 & 0.9787 \\
    \hline
    Segwa chouki II & Vadtalav PZ & 0.97647 & 0.97773 \\
    \hline
    \end{tabular}%
  \label{tab:table7_1}%
\end{table}%

